COMPASS: Unsupervised and Online Clustering of Complex Human Activities from Smartphone Sensors

Modern mobile devices are able to provide context-aware and personalized services to the users, by leveraging on their sensing capabilities to infer the activity and situation in which a person is currently involved. Current solutions for context-recognition rely on annotated data and expertsâ€™ knowledge to predict the user context. In addition, their prediction ability is strongly limited to the set of situations considered during the model training or definition. However, in a mobile environment, the user context continuously evolves, and it cannot be merely restricted to a set of predefined classes. To overcome these limitations, we propose COMPASS, a novel unsupervised and online clustering algorithm aimed at identifying the user context in mobile environments based on the stream of high-dimensional data generated by smartphone sensors. COMPASScan distinguish an arbitrary number of userâ€™s contexts from the sensorsâ€™ data, without defining a priori the collection of expected situations. This key feature makes it a general-purpose solution to provide context-aware features to mobile devices, supporting a broad set of applications. Experimental results on 18 synthetic and 2 real-world datasets show that COMPASS correctly identifies the user context from the sensorsâ€™ data stream, and outperforms the state-of-the-art solutions in terms of both clusters configuration and purity. Eventually, we evaluate its performances in terms of execution time and the results show that COMPASS can process 1000 high-dimensional samples in less than 20 seconds, while the reference solutions require about 60 minutes to evaluate the entire dataset. Keywords: Context-awareness, Unsupervised Machine Learning, Online Clustering, Mobile Computing

==> extrasensory_parameters.tex <==
\begin{table}[t]
\caption{Best parameters for the ExtraSensory Dataset.}
\begin{tabular}{cccc | cccc | ccc}
    \toprule
    \multicolumn{4}{c|}{\dbstream} &
    \multicolumn{4}{c|}{\dstream} &
    \multicolumn{3}{c}{\compass}
    \\ \midrule
    r       & $C_m$         & $\alpha$      & $t_{gap}$   &
    $g_s$   & $t_{gap}$     & $C_m$         & $C_l$       &
    $t_w$   & d             & k
    \\ \midrule
    10      & 6             & 0.1           & 100         &
    20      & 100           & 2             & 1           &
    600s    & 5             & 5   
    \\\bottomrule
\end{tabular}
\label{tab:extrasensory_parameters}
\end{table}
